MAUVE Scores for Generative Models: Theory and Practice

Generative artificial intelligence has made significant strides, producing text indistinguishable from human prose and remarkably photorealistic images. Automatically measuring how close the generated data distribution is to the target distribution is central to diagnosing existing models and developing better ones. We present MAUVE, a family of comparison measures between pairs of distributions such as those encountered in the generative modeling of text or images. These scores are statistical summaries of divergence frontiers capturing two types of errors in generative modeling. We explore three approaches to statistically estimate these scores: vector quantization, non-parametric estimation, and classifier-based estimation. We provide statistical bounds for the vector quantization approach. Empirically, we find that the proposed scores paired with a range of $f$-divergences and statistical estimation methods can quantify the gaps between the distributions of human-written text and those of modern neural language models by correlating with human judgments and identifying known properties of the generated texts. We demonstrate in the vision domain that MAUVE can identify known properties of generated images on par with or better than existing metrics. In conclusion, we present practical recommendations for using MAUVE effectively with language and image modalities.

==> tables/combined/beam_search.tex <==
\begin{tabular}{lccccccc}
\toprule
% {\bf Decoding}
% & Greedy & 
% \begin{tabular}{c} Beam \\ $b=4$ \end{tabular} 
% & \begin{tabular}{c} Beam $b=4$ + \\  no $4$-gram repeat \end{tabular} 
% &
% \begin{tabular}{c} Beam \\ $b=8$ \end{tabular} &
% \begin{tabular}{c} Beam $b=8$ + \\  no $4$-gram repeat \end{tabular} & 
% Ancestral & 
% Nucleus \\
\multirow{2}{*}{\textbf{Decoding}}
& \multirow{2}{*}{Greedy} & 
\multicolumn{2}{c}{Beam} 
& 
\multicolumn{2}{c}{Beam + no $4$-gram repeat}
& 
\multirow{2}{*}{Ancestral} & 
\multirow{2}{*}{Nucleus} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
& & $b=4$ & $b=8$ & $b=4$ & $b=8$ & & \\
\midrule
\bf \mauve & 
$0.008$ & 
$0.021$ & 
$0.026$ & 
$0.366$ & 
$0.341$ & 
$0.589_{0.02}$ & 
\tabemph{} $\mathbf{0.878_{0.007}}$  \\
\bottomrule
\end{tabular}

==> tables/combined/corr_discretization_new.tex <==
\begin{tabular}{lrr}
\toprule
\small
\bf Quantization & ${k}$ & \bf Corr. \\
\midrule
    DRMM    & - &  $0.99$ \\
    Lattice & - &  $0.99$ \\
\midrule[0.03em]
\multirow{5}{*}{$k$-means}
& $10$    &   $0.98$ \\
& $100$  &      $0.99$ \\
& $250$  &       $0.99$ \\
& $1000$ &      $1.00$ \\
& $5000$ &       $0.99$ \\
\bottomrule
\end{tabular}



% \begin{tabular}{llr}
% \toprule
% \bf Discretization & & \bf Correlation \\
% \midrule
%     DRMM    & &  $0.9896$ \\
%     Lattice & &  $0.9896$ \\
% \midrule[0.03em]
% \multirow{5}{*}{$k$-means} 
% & $k=10$    &   $0.9800$ \\
% % & $k=50$    &   $0.9956$ \\
% & $k=100$  &      $0.9939$ \\
% & $k=250$  &       $0.9921$ \\
% & $k=1000$ &      $0.9965$ \\
% % & $k=2000$ &       $0.9973$ \\
% & $k=5000$ &       $0.9895$ \\
% \bottomrule
% \end{tabular}

% \begin{tabular}{llr}
% \toprule
% \bf Discretization & & \bf Correlation \\
% \midrule
%     DRMM    & &  $0.97$ \\
%     Lattice & &  $0.93$ \\
% \midrule[0.03em]
% \multirow{5}{*}{$k$-means} & $k=100$  &      $0.94$ \\
% & $k=250$  &       $1.00$ \\
% & $k=1000$ &      $0.94$ \\
% & $k=1500$ &       $1.00$ \\
% & $k=2000$ &       $1.00$ \\
% \bottomrule
% \end{tabular}



==> tables/combined/corr_gold.tex <==
\begin{tabular}{llcccccc}
\toprule
\textbf{Metric} & \textbf{Task} & \textbf{Gen. PPL} & \textbf{Zipf Coef.} & \textbf{REP} & \textbf{Distinct-4} & \textbf{Self-BLEU} & \textbf{\name} \\
\midrule
       Human-like/BT &      Web text &           $0.810$ &             $0.762$ &     $-0.500$ &             $0.738$ &            $0.500$ &        \tabemph{$\mathbf{0.857}$} \\
      Interesting/BT &      Web text &           $0.643$ &             $0.405$ &     $-0.571$ &             $0.524$ &            $0.262$ &        \tabemph{$\mathbf{0.714}$} \\
         Sensible/BT &      Web text &           $0.738$ &             $0.643$ &     $-0.476$ &             $0.595$ &            $0.452$ &        \tabemph{$\mathbf{0.762}$} \\
      Disc. Acc. &          News &           $0.468$ &             $0.595$ &      $0.792$ &             $0.653$ &            $0.516$ &        \tabemph{$\mathbf{0.956}$} \\
       Disc. Acc. &       Stories &           $0.643$ &             $0.643$ &      $0.250$ &             $0.750$ &            $0.857$ &        \tabemph{$\mathbf{0.893}$} \\
\bottomrule
\end{tabular}



% \begin{tabular}{llrrrrrr}
% \toprule
% \textbf{Metric} & \textbf{Task} & \textbf{Gen. PPL} & \textbf{Zipf Coef.} & \textbf{REP} & \textbf{Distinct-4} & \textbf{Self-BLEU} & \textbf{\name} \\
% \midrule
%       Human-like/BT &      Web text &           $0.810$ &             $0.833$ &     $-0.167$ &             $0.738$ &            $0.595$ &        \tabemph{$\mathbf{0.952}$} \\
%       Interesting/BT &      Web text &           $0.643$ &             $0.524$ &     $-0.143$ &             $0.524$ &            $0.405$ &        \tabemph{$\mathbf{0.810}$} \\
%          Sensible/BT &      Web text &           $0.738$ &             $0.690$ &     $-0.071$ &             $0.595$ &            $0.524$ &        \tabemph{$\mathbf{0.857}$} \\
%       \% Disc. Acc. &          News &           $0.468$ &             $0.595$ &      $0.792$ &             $0.653$ &            $0.516$ &        \tabemph{$\mathbf{0.956}$} \\
%         \% Disc. Acc. &       Stories &           $0.643$ &             $0.643$ &      $0.250$ &             $0.750$ &            $0.857$ &        \tabemph{$\mathbf{0.893}$} \\
% \bottomrule
% \end{tabular}

==> tables/combined/corr_human_eval_all.tex <==
\begin{tabular}{ccccccc}
\toprule
{} & Gen. PPL & Zipf Coef. &       REP & Distinct-4 & Self-BLEU & \textsc{mauve} \\
\midrule
BT/Human-like  &  $0.810$ &    $0.833$ &  $-0.167$ &    $0.738$ &   $0.595$ &        \tabemph{$\mathbf{0.952}$} \\
BT/Interesting &  $0.643$ &    $0.524$ &  $-0.143$ &    $0.524$ &   $0.405$ &        \tabemph{$\mathbf{0.810}$} \\
BT/Sensible    &  $0.738$ &    $0.690$ &  $-0.071$ &    $0.595$ &   $0.524$ &        \tabemph{$\mathbf{0.857}$} \\
\bottomrule
\end{tabular}


==> tables/combined/decoding_model_two_table.tex <==
\begin{table}[t]
\RawFloats
\footnotesize
\begin{minipage}[t]{0.47\linewidth}
\setlength{\tabcolsep}{2pt}
\begin{center}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{rrrrr}
\toprule
& \textbf{Adv.}&\textbf{Greedy} & \textbf{Sampling} & \textbf{Nucleus} \\\midrule
\textbf{Gen. PPL}($\downarrow$) & \tabemph{$\mathbf{0.05}$} & $11.3$ & $19.3$ & $1.54$\\
\textbf{Zipf}($\downarrow$)& $0.03$ & $0.02$ & $0.02$ & \tabemph{$\mathbf{0.01}$}\\
\textbf{Self-BLEU}($\downarrow$)& $0.07$ & $0.03$ & \tabemph{$\mathbf{0.02}$} & $0.03$\\
 \bf   SP($\uparrow$) & -- & $0.50$ &\tabemph{$\mathbf{0.69}$} & $0.69$\\
 \bf JS($\downarrow$) &-- & \tabemph{$\mathbf{0.35}$} & $0.37$ & $0.36$\\
 \bf $\epsilon$-PPL($\downarrow$) & --& $497$ & \tabemph{$\mathbf{11.4}$}  & $13.7$\\
\bf \name($\uparrow$) & $0.06$ & $0.02$ & $0.88$ & \tabemph{$\mathbf{0.94}$}\\\hline
 \bf Human($\uparrow$) & --& -- & $9.0$ & \tabemph{$\mathbf{15.7}$}\\
 \bottomrule
\addlinespace[0.4em] 
\end{tabular}
}
\caption{ \small 
Generation quality w.r.t\ different \textbf{decoding algorithms} (web text, GPT-2 xl) under various metrics, and humans. 
\name correctly captures the relationship $\text{greedy}\prec\text{ancestral}\prec{\text{nucleus}}$, and rates the adversarial decoder's text as low quality.
Results are consistent across model sizes and random seeds. % (Appendix~\autoref{}).
Boldfaced/highlighted entries denote the best decoding algorithm under each metric.
% greatest similarity between the model and human distributions per each measure.
}
\label{tbl:decoding}
\end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{.47\linewidth}
\setlength{\tabcolsep}{3pt}
\begin{center}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{rrrrr}
\toprule
& \textbf{Small}&\textbf{Medium} & \textbf{Large} & \textbf{XL} \\\midrule
\textbf{Gen. PPL}($\downarrow$) & $11.2$ & $8.5$ & \tabemph{$\mathbf{0.9}$} & $1.5$\\
\textbf{Zipf}($\downarrow$) & $0.06$ & \tabemph{$\mathbf{0.00}$} & $0.02$ & $0.01$\\
\textbf{Self-BLEU}($\downarrow$) & $0.05$ & \tabemph{$\mathbf{0.02}$} & $0.03$ & $0.03$\\
 \bf   SP($\uparrow$) &  $0.65$ & $0.67$ & $0.68$ & \tabemph{$\mathbf{0.69}$}\\
 \bf JS($\downarrow$) & $0.41$ & $0.39$ & $0.37$ & \tabemph{$\mathbf{0.36}$}\\
 \bf $\epsilon$-PPL($\downarrow$) & $25.9$ & $18.8$ & $14.9$ & \tabemph{$\mathbf{13.7}$}\\
 \bf \name($\uparrow$) & $0.878$ & $0.915$ & $0.936$ & \tabemph{$\mathbf{0.940}$}\\\hline
 \bf Human($\uparrow$) & $-15.9$ & $-3.4$ & $12.6$ & \tabemph{$\mathbf{15.7}$}\\
 \bottomrule
\addlinespace[0.4em] 
\end{tabular}
}
\caption{\small
Generation quality w.r.t\ different \textbf{model sizes} (web text, nucleus sampling) under various metrics, as well as human evaluators.
\name captures the relationship between model size and generation quality, agreeing with human-evaluated quality.
Results are consistent across random seeds and decoding algorithms. % (Appendix~\autoref{})
Boldfaced/highlighted entries denote the best model size under each metric.
% the greatest similarity between the 
% model and human distributions per each measure.
}
\label{tbl:modelsize}
\end{center}
\end{minipage}
\end{table}




==> tables/combined/human_eval_all.tex <==
\begin{tabular}{ccrrr}
\toprule
  \textbf{GPT-2 Size}    &  \textbf{Decoding}  & \textbf{BT/Human-like} & \textbf{BT/Interesting} & \textbf{BT/Sensible} \\
\midrule
Human & {} &      $47.251$ &       $25.503$ &    $43.229$ \\
\hline
xl & Nucleus, $p=0.95$ &      \tabemph{$\mathbf{15.664}$} &       \tabemph{$\mathbf{23.046}$} &    \tabemph{$\mathbf{31.888}$} \\
      & Sampling &       $8.966$ &        $9.529$ &     $7.753$ \\
\hline
large & Nucleus, $p=0.95$ &      $12.553$ &        $6.785$ &     $8.781$ \\
      & Sampling &      $-6.935$ &       $-1.532$ &    $-7.106$ \\
\hline
medium & Nucleus, $p=0.9$ &      $-3.429$ &      $-12.824$ &    $-7.293$ \\
      & Sampling &     $-30.769$ &      $-34.323$ &   $-32.004$ \\
\hline
small & Nucleus, $p=0.9$ &     $-15.783$ &       $-0.697$ &    $-7.442$ \\
      & Sampling &     $-27.518$ &      $-15.487$ &   $-37.805$ \\
\bottomrule
\end{tabular}


==> tables/combined/main_std_new_prefix.tex <==
\begin{tabular}{lllllllrrrrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &      \bf              Gen. PPL &           \bf     Zipf Coef. &               \bf        Rep. &       \bf         Distinct-4 &           \bf      Self-BLEU & \bf   SP($\uparrow$) &  \bf JS($\downarrow$) & \bf $\epsilon$-PPL($\downarrow$) & \bf Human/BT($\uparrow$) & \bf \textsc{mauve}($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Sampling &          $101.880_{0.627}$ &           $0.926_{0.001}$ &           $0.001_{0.000}$ &           $0.941_{0.001}$ &           $0.327_{0.003}$ &           $0.653$ &           $0.425$ &                     $19.401$ &             $-27.52$ &            $0.589_{0.018}$ \\
      & Greedy &                    $1.224$ &                   $1.037$ &                   $0.942$ &                   $0.072$ &           $0.465_{0.000}$ &           $0.431$ &           $0.394$ &                   $1049.589$ &          --            &                    $0.008$ \\
      & Nucleus, $0.9$ &           $23.788_{0.144}$ &           $1.012_{0.002}$ &           $0.010_{0.001}$ &           $0.859_{0.002}$ &           $0.436_{0.004}$ &           $0.652$ &           $0.414$ &                     $25.938$ &             $-15.78$ &            $0.878_{0.006}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $1.073$ &           $0.006$ &           $0.365$ &           $0.525$ &       -- &           -- &                     -- &             -- &            $0.043$ \\
\midrule
\multirow{4}{*}{medium} & Sampling &          $129.263_{0.798}$ &           $0.872_{0.001}$ &           $0.001_{0.000}$ &           $0.953_{0.001}$ &           $0.281_{0.002}$ &           $0.670$ &           $0.402$ &                     $14.631$ &             $-30.77$ &            $0.373_{0.010}$ \\
      & Greedy &                    $1.241$ &                   $0.978$ &                   $0.903$ &                   $0.091$ &                   $0.415$ &           $0.465$ &           $0.371$ &                    $708.057$ &              --        &                    $0.012$ \\
      & Nucleus, $0.9$ &           $21.073_{0.134}$ &           \tabemph{$\mathbf{0.957}_{0.001}$} &           $0.005_{0.001}$ &  \tabemph{$\mathbf{0.884}_{0.001}$} &  \tabemph{$\mathbf{0.402}_{0.003}$} &           $0.670$ &           $0.391$ &                     $18.821$ &              $-3.43$ &            $0.915_{0.006}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $1.006$ &           $0.005$ &           $0.381$ &           $0.444$ &       -- &           -- &                     -- &             -- &            $0.044$ \\
\midrule
\multirow{4}{*}{large} & Sampling &           $30.080_{0.196}$ &           $0.930_{0.002}$ &  \tabemph{$\mathbf{0.002}_{0.001}$} &           $0.916_{0.001}$ &           $0.358_{0.001}$ &           $0.679$ &           $0.381$ &                     $12.658$ &              $-6.93$ &            $0.845_{0.010}$ \\
      & Greedy &                    $1.232$ &                   $0.983$ &                   $0.881$ &                   $0.100$ &                   $0.413$ &           $0.483$ &           $0.359$ &                    $580.020$ &            --          &                    $0.012$ \\
      & Nucleus, $0.95$ &  $13.499_{0.058}$ &  $0.967_{0.002}$ &           $0.006_{0.001}$ &           $0.870_{0.001}$ &           $0.412_{0.002}$ &           $0.679$ &           $0.374$ &                     $14.938$ &              $12.55$ &            $0.936_{0.003}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.965$ &           $0.005$ &           $0.395$ &           $0.429$ &       -- &           -- &                     -- &             -- &            $0.035$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Sampling &           $31.886_{0.447}$ &           $0.930_{0.001}$ &           $0.002_{0.001}$ &           $0.913_{0.001}$ &           $0.360_{0.003}$ &  \tabemph{$\mathbf{0.686}$} &           $0.369$ &            \tabemph{$\mathbf{11.412}$} &               $8.97$ &            $0.882_{0.006}$ \\
      & Greedy &                    $1.278$ &                   $0.975$ &                   $0.859$ &                   $0.115$ &                   $0.417$ &           $0.496$ &  \tabemph{$\mathbf{0.349}$} &                    $497.696$ &              --        &                    $0.016$ \\
      & Nucleus, $0.95$ &           $14.143_{0.043}$ &           $0.966_{0.002}$ &           $0.005_{0.000}$ &           $0.868_{0.001}$ &           $0.413_{0.002}$ &           $0.686$ &           $0.363$ &                     $13.677$ &     \tabemph{$\mathbf{15.66}$} &   \tabemph{$\mathbf{0.940}_{0.006}$} \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.986$ &           $0.005$ &           $0.397$ &           $0.448$ &       -- &           -- &                     -- &             -- &            $0.057$ \\
\midrule
Human &         n/a          &                   $12.602$ &                   $0.952$ &                   $0.002$ &                   $0.878$ &                   $0.382$ &        --           &        --           &             --                 &              $47.25$ &            --                \\
\bottomrule
\end{tabular}


==> tables/combined/typical_decoding.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{
\textbf{Decoding}
}
& 
\multicolumn{6}{c}{Locally Typical Sampling}
& \multirow{2}{*}{Nucleus}\\
\cmidrule{2-7}
&
$p=0.2$ & $p=0.5$ & $p=0.7$ & $p=0.9$ & $p=0.95$ & $p=0.99$ &  
 \\
\midrule
\bf \mauve & 
$0.826_{0.014}$ & 
$0.868_{0.007}$ & 
$0.850_{0.012}$ & 
$0.920_{0.011}$ & 
\tabemph{} $\mathbf{0.933_{0.007}}$ & 
$0.889_{0.009}$ & 
\tabemph{} $\mathbf{0.936_{0.004}}$  \\
\bottomrule
\end{tabular}

==> tables/combined/webtext_full_LM.tex <==
\begin{tabular}{llrrrrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &  \bf   SP($\uparrow$) &  \bf JS($\downarrow$) & \bf $\epsilon$-PPL($\downarrow$) & \bf Human/BT($\uparrow$) & \bf \name($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Greedy &                         $0.431$ &           $0.394$ &                   $1049.589$ &          --            &                    $0.008$ \\
& Sampling &             $0.653$ &           $0.425$ &                     $19.401$ &             $-27.52$ &            $0.589_{0.018}$ \\
      & Nucleus, $0.9$ &         $0.652$ &           $0.414$ &                     $25.938$ &             $-15.78$ &            $0.878_{0.006}$ \\
\midrule
\multirow{4}{*}{medium} & Greedy &                          $0.465$ &           $0.371$ &                    $708.057$ &              --        &                    $0.012$ \\
& Sampling &      $0.670$ &           $0.402$ &                     $14.631$ &             $-30.77$ &            $0.373_{0.010}$ \\
      & Nucleus, $0.9$ &              $0.670$ &           $0.391$ &                     $18.821$ &              $-3.43$ &            $0.915_{0.006}$ \\
\midrule
\multirow{4}{*}{large} & Greedy &                     $0.483$ &           $0.359$ &                    $580.020$ &            --          &                    $0.012$ \\
& Sampling &     $0.679$ &           $0.381$ &                     $12.658$ &              $-6.93$ &            $0.845_{0.010}$ \\
      & Nucleus, $0.95$ &    $0.679$ &           $0.374$ &                     $14.938$ &              $12.55$ &            $0.936_{0.003}$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Greedy &                      $0.496$ &  \tabemph{$\mathbf{0.349}$} &                    $497.696$ &              --        &                    $0.016$ \\
    & Sampling &      \tabemph{$\mathbf{0.686}$} &           $0.369$ &            \tabemph{$\mathbf{11.412}$} &               $8.97$ &            $0.882_{0.006}$ \\
      & Nucleus, $0.95$ &            $0.686$ &           $0.363$ &                     $13.677$ &    \tabemph{$\mathbf{15.66}$} &   \tabemph{$\mathbf{0.940}_{0.006}$} \\
      & Adversarial &           n/a &           n/a &                     n/a &             -- &            $0.057$ \\
\bottomrule
\end{tabular}


==> tables/combined/webtext_full_ref.tex <==
\begin{tabular}{lllllllrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &      \bf              Gen. PPL &           \bf     Zipf Coef. &               \bf        Rep. &       \bf         Distinct-4 &           \bf      Self-BLEU & \bf Human($\uparrow$) & \bf \name($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Sampling &          $101.880_{0.627}$ &           $0.926_{0.001}$ &           $0.001_{0.000}$ &           $0.941_{0.001}$ &           $0.327_{0.003}$ &                      $-27.52$ &            $0.589_{0.018}$ \\
      & Greedy &                    $1.224$ &                   $1.037$ &                   $0.942$ &                   $0.072$ &           $0.465_{0.000}$ &                 --            &                    $0.008$ \\
      & Nucleus, $0.9$ &           $23.788_{0.144}$ &           $1.012_{0.002}$ &           $0.010_{0.001}$ &           $0.859_{0.002}$ &           $0.436_{0.004}$ &              $-15.78$ &            $0.878_{0.006}$ \\
      & Adversarial &            \tabemph{$\mathbf{12.554}$} &           $1.073$ &           $0.006$ &           $0.365$ &           $0.525$ &             -- &            $0.043$ \\
\midrule
\multirow{4}{*}{medium} & Sampling &          $129.263_{0.798}$ &           $0.872_{0.001}$ &           $0.001_{0.000}$ &           $0.953_{0.001}$ &           $0.281_{0.002}$ &              $-30.77$ &            $0.373_{0.010}$ \\
      & Greedy &                    $1.241$ &                   $0.978$ &                   $0.903$ &                   $0.091$ &                   $0.415$ &                 --        &                    $0.012$ \\
      & Nucleus, $0.9$ &           $21.073_{0.134}$ &           \tabemph{$\mathbf{0.957}_{0.001}$} &           $0.005_{0.001}$ &  \tabemph{$\mathbf{0.884}_{0.001}$} &  \tabemph{$\mathbf{0.402}_{0.003}$} &                  $-3.43$ &            $0.915_{0.006}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $1.006$ &           $0.005$ &           $0.381$ &           $0.444$ &            -- &            $0.044$ \\
\midrule
\multirow{4}{*}{large} & Sampling &           $30.080_{0.196}$ &           $0.930_{0.002}$ &  \tabemph{$\mathbf{0.002}_{0.001}$} &           $0.916_{0.001}$ &           $0.358_{0.001}$ &                $-6.93$ &            $0.845_{0.010}$ \\
      & Greedy &                    $1.232$ &                   $0.983$ &                   $0.881$ &                   $0.100$ &                   $0.413$ &       --          &                    $0.012$ \\
      & Nucleus, $0.95$ &  $13.499_{0.058}$ &  $0.967_{0.002}$ &           $0.006_{0.001}$ &           $0.870_{0.001}$ &           $0.412_{0.002}$ &             $12.55$ &            $0.936_{0.003}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.965$ &           $0.005$ &           $0.395$ &           $0.429$ &        -- &            $0.035$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Sampling &           $31.886_{0.447}$ &           $0.930_{0.001}$ &           $0.002_{0.001}$ &           $0.913_{0.001}$ &           $0.360_{0.003}$ &            $8.97$ &            $0.882_{0.006}$ \\
      & Greedy &                    $1.278$ &                   $0.975$ &                   $0.859$ &                   $0.115$ &                   $0.417$ &               --        &                    $0.016$ \\
      & Nucleus, $0.95$ &           $14.143_{0.043}$ &           $0.966_{0.002}$ &           $0.005_{0.000}$ &           $0.868_{0.001}$ &           $0.413_{0.002}$ &      \tabemph{$\mathbf{15.66}$} &   \tabemph{$\mathbf{0.940}_{0.006}$} \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.986$ &           $0.005$ &           $0.397$ &           $0.448$ &      -- &            $0.057$ \\
\midrule
Human &         n/a          &                   $12.602$ &                   $0.952$ &                   $0.002$ &                   $0.878$ &                   $0.382$ &         $47.25$ &            --                \\
\bottomrule
\end{tabular}

==> tables/combined/webtext_main_old.tex <==
\begin{tabular}{lllllllrrrrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &      \bf              Gen. PPL &           \bf     Zipf Coef. &               \bf        Rep. &       \bf         Distinct-4 &           \bf      Self-BLEU & \bf   SP($\uparrow$) &  \bf JS($\downarrow$) & \bf $\epsilon$-PPL($\downarrow$) & \bf Human/BT($\uparrow$) & \bf \textsc{mauve}($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Sampling &          $101.880_{0.627}$ &           $0.926_{0.001}$ &           $0.001_{0.000}$ &           $0.941_{0.001}$ &           $0.327_{0.003}$ &           $0.653$ &           $0.425$ &                     $19.401$ &             $-27.52$ &            $0.589_{0.018}$ \\
      & Greedy &                    $1.224$ &                   $1.037$ &                   $0.942$ &                   $0.072$ &           $0.465_{0.000}$ &           $0.431$ &           $0.394$ &                   $1049.589$ &          --            &                    $0.008$ \\
      & Nucleus, $0.9$ &           $23.788_{0.144}$ &           $1.012_{0.002}$ &           $0.010_{0.001}$ &           $0.859_{0.002}$ &           $0.436_{0.004}$ &           $0.652$ &           $0.414$ &                     $25.938$ &             $-15.78$ &            $0.878_{0.006}$ \\
      & Adversarial &           $\mathbf{12.554}$ &           $1.073$ &           $0.006$ &           $0.365$ &           $0.525$ &       -- &           -- &                     -- &             -- &            $0.043$ \\
\midrule
\multirow{4}{*}{medium} & Sampling &          $129.263_{0.798}$ &           $0.872_{0.001}$ &           $0.001_{0.000}$ &           $0.953_{0.001}$ &           $0.281_{0.002}$ &           $0.670$ &           $0.402$ &                     $14.631$ &             $-30.77$ &            $0.373_{0.010}$ \\
      & Greedy &                    $1.241$ &                   $0.978$ &                   $0.903$ &                   $0.091$ &                   $0.415$ &           $0.465$ &           $0.371$ &                    $708.057$ &              --        &                    $0.012$ \\
      & Nucleus, $0.9$ &           $21.073_{0.134}$ &           $\mathbf{0.957}_{0.001}$ &           $0.005_{0.001}$ &  $\mathbf{0.884}_{0.001}$ &  $\mathbf{0.402}_{0.003}$ &           $0.670$ &           $0.391$ &                     $18.821$ &              $-3.43$ &            $0.915_{0.006}$ \\
      & Adversarial &           $\mathbf{12.554}$ &           $1.006$ &           $0.005$ &           $0.381$ &           $0.444$ &       -- &           -- &                     -- &             -- &            $0.044$ \\
\midrule
\multirow{4}{*}{large} & Sampling &           $30.080_{0.196}$ &           $0.930_{0.002}$ &  $\mathbf{0.002}_{0.001}$ &           $0.916_{0.001}$ &           $0.358_{0.001}$ &           $0.679$ &           $0.381$ &                     $12.658$ &              $-6.93$ &            $0.845_{0.010}$ \\
      & Greedy &                    $1.232$ &                   $0.983$ &                   $0.881$ &                   $0.100$ &                   $0.413$ &           $0.483$ &           $0.359$ &                    $580.020$ &            --          &                    $0.012$ \\
      & Nucleus, $0.95$ &  $13.499_{0.058}$ &  $0.967_{0.002}$ &           $0.006_{0.001}$ &           $0.870_{0.001}$ &           $0.412_{0.002}$ &           $0.679$ &           $0.374$ &                     $14.938$ &              $12.55$ &            $0.936_{0.003}$ \\
      & Adversarial &           $\mathbf{12.554}$ &           $0.965$ &           $0.005$ &           $0.395$ &           $0.429$ &       -- &           -- &                     -- &             -- &            $0.035$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Sampling &           $31.886_{0.447}$ &           $0.930_{0.001}$ &           $0.002_{0.001}$ &           $0.913_{0.001}$ &           $0.360_{0.003}$ &  $\mathbf{0.686}$ &           $0.369$ &            $\mathbf{11.412}$ &               $8.97$ &            $0.882_{0.006}$ \\
      & Greedy &                    $1.278$ &                   $0.975$ &                   $0.859$ &                   $0.115$ &                   $0.417$ &           $0.496$ &  $\mathbf{0.349}$ &                    $497.696$ &              --        &                    $0.016$ \\
      & Nucleus, $0.95$ &           $14.143_{0.043}$ &           $0.966_{0.002}$ &           $0.005_{0.000}$ &           $0.868_{0.001}$ &           $0.413_{0.002}$ &           $0.686$ &           $0.363$ &                     $13.677$ &     $\mathbf{15.66}$ &   $\mathbf{0.940}_{0.006}$ \\
      & Adversarial &           $\mathbf{12.554}$ &           $0.986$ &           $0.005$ &           $0.397$ &           $0.448$ &       -- &           -- &                     -- &             -- &            $0.057$ \\
\midrule
Human &         n/a          &                   $12.602$ &                   $0.952$ &                   $0.002$ &                   $0.878$ &                   $0.382$ &        --           &        --           &             --                 &              $47.25$ &            --                \\
\bottomrule
\end{tabular}


==> tables/combined/wp_std.tex <==
\begin{tabular}{llllllll}
\toprule
\textbf{Decoding} &                   \textbf{Gen. PPL} &                \textbf{Zipf Coef.} &                       \textbf{REP} &                \textbf{Distinct-4} &                 \textbf{Self-BLEU} & \textbf{\% Disc. Acc. ($\downarrow$)} & \textbf{\textsc{mauve}($\uparrow$)} \\
\midrule
Sampling          &           $38.983_{0.143}$ &  \tabemph{$\mathbf{1.066}_{0.002}$} &  \tabemph{$\mathbf{0.001}_{0.000}$} &           $0.833_{0.001}$ &           $0.518_{0.003}$ &              $78.1_{0.4}$ &            $0.905_{0.010}$ \\
Nucleus, $0.9$  &           $15.433_{0.042}$ &           $1.201_{0.002}$ &           $0.006_{0.001}$ &           $0.719_{0.001}$ &           $0.637_{0.002}$ &              $75.2_{0.4}$ &            $0.887_{0.008}$ \\
Nucleus, $0.92$ &           $17.422_{0.060}$ &           $1.179_{0.002}$ &           $0.004_{0.001}$ &           $0.742_{0.001}$ &           $0.620_{0.003}$ &              $72.0_{0.6}$ &            $0.901_{0.005}$ \\
Nucleus, $0.95$ &  \tabemph{$\mathbf{21.599}_{0.127}$} &           $1.147_{0.002}$ &           $0.003_{0.000}$ &  \tabemph{$\mathbf{0.775}_{0.002}$} &           $0.589_{0.005}$ &     \tabemph{$\mathbf{68.6}_{0.6}$} &   \tabemph{$\mathbf{0.920}_{0.004}$} \\
Top-$100$  &           $16.527_{0.041}$ &           $1.252_{0.001}$ &           $0.002_{0.000}$ &           $0.743_{0.001}$ &           $0.631_{0.001}$ &              $78.2_{0.2}$ &            $0.884_{0.007}$ \\
Top-$500$  &           $23.833_{0.076}$ &           $1.153_{0.001}$ &           $0.001_{0.000}$ &           $0.794_{0.001}$ &  \tabemph{$\mathbf{57.6}_{0.2}$} &              $0.697_{0.005}$ &            $0.919_{0.005}$ \\
Greedy            &                    $1.739$ &                   $1.362$ &                   $0.988$ &                   $0.101$ &                   $0.742$ &                      $99.7$ &                    $0.005$ \\
\midrule
Human             &                   $19.704$ &                   $1.101$ &                   $0.001$ &                   $0.783$ &                   $0.571$ &                              &                            \\
\bottomrule
\end{tabular}


==> tables/grover/discr_correlation.tex <==
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\bf Discriminator}
& \multicolumn{2}{c}{BERT}
& \multicolumn{3}{c}{GPT-2}
& \multicolumn{3}{c}{Grover} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
& Base & Large & Small & Medium & Large & Base & Large & Mega \\
\midrule
\bf Correlation & 0.803 & 0.817 & 0.831 & 0.829 & 0.822 & 0.928 & 0.956 & 0.925 \\
\bottomrule
\end{tabular}


% \begin{tabular}{llr}
% \toprule
% \bf Discriminator & \bf Size & \bf Correlation \\
% \midrule
% \multirow{2}{*}{BERT} & base    &       0.803 \\
% & large   &       0.817 \\
% \midrule
% \multirow{2}{*}{GPT-2} & small  &       0.831 \\
% & medium &       0.829 \\
% & large &       0.822 \\
% \midrule
% \multirow{3}{*}{Grover} & base  &       0.928 \\
% & large &       0.956 \\
% & mega  &       0.925 \\
% \bottomrule
% \end{tabular}


==> tables/grover/main_grover.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
\bf Grover Size      &    \bf  Decoding              &       \bf     Gen. PPL &     \bf    Zipf Coef. &     \bf           Rep. &    \bf     Distinct-4 &      \bf    Self-BLEU &  \bf \% Disc. Acc.($\downarrow$) & \bf \textsc{mauve}($\uparrow$) \\
\midrule
\multirow{3}{*}{base} & Sampling &           $37.505$ &           $0.942$ &           $0.002$ &           $0.882$ &           $0.419$ &                     $99.925$ &                    $0.700$ \\
      & Greedy &            $1.413$ &           $1.038$ &           $0.518$ &           $0.081$ &           $0.548$ &                    $100.000$ &                    $0.005$ \\
      & Nucleus, $0.96$ &           $23.064$ &           $0.974$ &           $0.006$ &  \tabemph{$\mathbf{0.847}$} &           $0.462$ &                     $99.950$ &                    $0.701$ \\
\midrule[0.03em]
\multirow{3}{*}{large} & Sampling &           $27.796$ &  ${0.946}$ &  \tabemph{$\mathbf{0.002}$} &           $0.878$ &           $0.429$ &                     $99.450$ &                    $0.794$ \\
      & Greedy &            $1.575$ &           $1.012$ &           $0.366$ &           $0.124$ &           $0.504$ &                    $100.000$ &                    $0.005$ \\
      & Nucleus, $0.98$ &           $20.792$ &           \tabemph{$\mathbf{0.962}$} &           $0.002$ &           $0.859$ &           $0.450$ &                     $98.475$ &                    $0.750$ \\
\midrule[0.03em]
\multirow{3}{*}{mega} & Sampling &           $22.656$ &           $0.950$ &           $0.001$ &           $0.879$ &           $0.427$ &                     $97.300$ &                    $0.808$ \\
      & Greedy &            $1.796$ &           $1.003$ &           $0.316$ &           $0.176$ &           $0.500$ &                    $100.000$ &                    $0.005$ \\
      & Nucleus, $0.96$ &  \tabemph{$\mathbf{14.834}$} &           $0.972$ &           $0.003$ &           $0.848$ &  \tabemph{$\mathbf{0.469}$} &            \tabemph{$\mathbf{88.675}$} &           \tabemph{$\mathbf{0.813}$} \\
\midrule
Human &      n/a             &           $15.356$ &           $0.956$ &           $0.002$ &           $0.842$ &           $0.473$ &         --                     &        --                    \\
\bottomrule
\end{tabular}


==> tables/hyperparam/featurizing_model.tex <==
\begin{tabular}{llcc}
\toprule
GPT-2 size         &     Decoding               &  
RoBERTa   &  GPT-2    \\
\midrule
small & Sampling &    0.174 &  0.589 \\
         & Greedy &   0.056 & 0.008 \\
         & Nucleus, $0.9$ &    0.723 &  0.878 \\
\midrule
medium & Sampling &    0.292 &   0.372 \\
         & Greedy &    0.114 & 0.011 \\
         & Nucleus, $0.9$ &    0.891 &  0.915 \\
\midrule
large & Sampling &    0.684 &  0.845 \\
         & Greedy &    0.125 & 0.012 \\
         & Nucleus, $0.95$ &     0.920 &  0.936 \\
\midrule
xl & Sampling &     0.780 &  0.881 \\
         & Greedy &     0.170 & 0.016 \\
         & Nucleus, $0.95$ &    \tabemph{\textbf{0.947}} &  \tabemph{\textbf{0.940}} \\
\bottomrule
\end{tabular}

==> tables/main/tab_decoding_strategies.tex <==
\begin{table*}[t!]
\tiny
\centering
\begin{tabular}{lclp{5cm}}
\toprule
Decoding  Algorithm 
& Type          & Parameters & 
$[\sigma(\pi)]_j$ definition (upto normalization)
   \\ \midrule
Pure Sampling      & Sampling      & -          & $\pi_j$                                     \\
Top-$K$~\citep{fan2018heirarchical} &
  Sampling &
  Integer $K$ &
  $\pi_j \, \mathbb{I}(j \in \mathrm{arg\,top\,k}_K(\pi))$ 
   \\
Nucleus~\citep{holtzman2019curious} &
  Sampling &
  $\rho \in (0, 1)$ &
  $\pi_j \, \mathbb{I}(j \in \mathrm{arg\,top\,prob}_\rho(\pi))$ 
   \\ 
 Consistent  Top-$K$~\cite{welleck2020consistency}
 &
  Sampling &
  Integer $K$ &
  $\pi_j \, \mathbb{I}(j \in \mathrm{arg\,top\,k}_K(\pi) \cup \{j_{\mathrm{eos}}\})$ 
   \\
Consistent  Nucleus~\cite{welleck2020consistency} 
&
  Sampling &
  $\rho \in (0, 1)$ &
  $\pi_j \, \mathbb{I}(j \in \mathrm{arg\,top\,prob}_\rho(\pi) \cup \{j_{\mathrm{eos}}\})$ 
   \\
Sparsemax~\citep{martins2020sparse} 
&
  Sampling 
  &
  - 
& $\pi_j$, where $p(\cdot | y_{<t}, x)$ is  parameterized differently 
  \\
Greedy             
& Deterministic & -          
& $\mathbb{I} (j \in \argmax_{i} \pi_i)$          
\\
Beam Search        
& Deterministic 
& -          
& See Text 
\\ 
Delayed Beam Search \citep{massarelli2019decoding} 
&
Sampling & Prefix length $L$  
& $\pi_j$, where
Sampling for $L$ steps followed by beam search \\ 
\bottomrule
\end{tabular}%
\caption{A survey of different decoding algorithms used in sampling.}
\label{tab:nlp:decoding-survey}
\end{table*}

==> tables/main/tab_evaluation_strategies.tex <==
\begin{table*}[t]
\centering
\tiny
% \begin{adjustbox}{max width=\textwidth}
% {\def\arraystretch{2}\tabcolsep=10pt
% \resizebox{\textwidth}{!}{%
\begin{tabular}{p{1cm}p{2cm}p{3cm}p{6cm}}
\toprule
\bf Type & \bf Metric &   \bf What does it measure?  &   \bf Limitations \\
\midrule
\multirow{6}{1cm}{Statistics based} &
Generation Perplexity
\citep{fan2018heirarchical,holtzman2019curious} &
Likelihood of text under model 
 &
Rewards low diversity generations like repetitions \\
& Zipf Coefficient
\citep{holtzman2019curious}
&
Unigram rank-frequency statistics
 &
Measures some properties of generated text, but is not stand-alone\\
& Self-BLEU 
   \citep{zhu2018texygen} &
  Diversity of  generation 
 &
Similar to BLEU, can only measure against a fixed number of references   \\
& Repetition Frequency \citep{holtzman2019curious,welleck2020neural} & 
Repetitiveness of generation 
 &
Can only measure a single property \\
& Non-termination Ratio
\citep{welleck2020consistency} &
Consistency 
&
\\
& Verifiability
   \citep{massarelli2019decoding} &
  Verifiability precision and recall 
 &
Can only measure a single property   \\
% Support per generation &
%   \citep{massarelli2019decoding} &
%   Verifiability recall &
%  &
% Can only measure a single property   \\
% Support per verified &
% \citep{massarelli2019decoding} &
% Verifiability precision &
%  &
% Can only measure a single property\\
\midrule[0.03em]
% Unique next-token &
%   \citep{welleck2020neural} &
%   Repetitiveness of argmax token &
%   &
%   \checkmark \\
\multirow{3}{1.5cm}{Language Modeling} &
$\epsilon$-perplexity
\citep{martins2020sparse} &
Perplexity with Laplace smoothing &
\multirow{3}{6cm}{Cannot be applied to deterministic decoding methods e.g. beam search.
Tend to reward text generated via pure sampling and greedy decoding, even if ``degenerate'' \cite{holtzman2019curious}} \\
& Sparsemax Score
\citep{martins2020sparse} &
LM quality via sparsemax loss~\cite{martins2016softmax}
& 
 \\
& JS Divergence (token-level)
\citep{martins2020sparse} &
LM quality using JS divergence
% reduction of uncertainty in the model distribution wrt samples of human text 
& 
\\
\midrule[0.03em]
\multicolumn{2}{c}{\name (this work)} &
Generation quality and diversity &
See \S\todo{\ref{}}\\
\bottomrule
\end{tabular}
\caption{
\small
Summary of automated metrics for evaluating open-ended text generation. 
Classical metrics (such as BLEU~\citep{papineni2002bleu}) which are task-specific and unsuitable for open-ended generation, as well as metrics specific to particular domains such as story generation have been omitted. 
}
\label{tab:nlp:auto-metrics-survey}
% }
% \end{adjustbox}
\end{table*}












% \begin{table*}[t]
% \centering
% \tiny
% % \begin{adjustbox}{max width=\textwidth}
% % {\def\arraystretch{2}\tabcolsep=10pt
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{p{2cm}lp{4cm}p{1.5cm}p{4cm}}
% \toprule
% \bf Metric &  \bf References &   \bf Measures &  \bf Type &   \bf Limitations \\
% \midrule
% Generation Perplexity &
% \citep{fan2018heirarchical,holtzman2019curious} &
% Plausibility of generation; based on likelihood of generations under the original $Q$ from the LM &
% \multirow{7}{1.5cm}{Model Distribution on Model Text} &
% Rewards low diversity generations like repetitions \\
% Zipf Coefficient &
% \citep{holtzman2019curious}
% &
% Word usage statistics, quantifies elationship between the frequency of words and their rank &
%  &
% Measures some properties of generated text, but is not stand-alone\\
% Self-BLEU &
%   \citep{zhu2018texygen} &
%   Diversity of  generation &
%  &
% Similar to BLEU, can only measure against a fixed number of references   \\
% Repetition Frequency
% & \citep{holtzman2019curious,welleck2020neural} & 
% Repetitiveness of generation & 
%  &
% Can only measure a single property \\
% Non-termination Ratio &
% \citep{welleck2020consistency} &
% Consistency &
% &
%   \\
% Support per generation &
%   \citep{massarelli2019decoding} &
%   Verifiability recall &
%  &
% Can only measure a single property   \\
% Support per verified &
% \citep{massarelli2019decoding} &
% Verifiability precision &
%  &
% Can only measure a single property\\
% \midrule[0.03em]
% % Unique next-token &
% %   \citep{welleck2020neural} &
% %   Repetitiveness of argmax token &
% %   &
% %   \checkmark \\
% $\epsilon$-perplexity &
% \citep{martins2020sparse} &
% LM quality via perplexity of human text after adding a Laplace smoothing to $Q$ &
% \multirow{3}{1.5cm}{Recalibrated Model Distribution on Reference Text}   &
% \multirow{6}{4cm}{Cannot be applied to deterministic decoding methods e.g. beam search.
% Tend to reward text generated via pure sampling and greedy decoding, even if ``degenerate'' \cite{holtzman2019curious}} \\
% Sparsemax Score &
% \citep{martins2020sparse} &
% quality of human text after the application of the entmax transformation \cite{peters2019sparse} to $Q$ &
%   &
%  \\
% JS Divergence &
% \citep{martins2020sparse} &
% reduction of uncertainty in the model distribution wrt samples of human text &
%   &
% \\
% \midrule[0.03em]
% \name &
% This Work &
% Generation quality and diversity &
% Model \& Human &
% See \S\todo{\ref{}}\\
% \bottomrule
% \end{tabular}
% \caption{Summary of automated metrics for evaluating open-ended text generation. 
% Classical metrics (such as BLEU; \citealp{papineni2002bleu}) which are task-specific and unsuitable for open-ended generation, as well as metrics specific to particular domains such as story generation have been omitted. 
% }
% \label{tab:nlp:auto-metrics-survey}
% % }
% % \end{adjustbox}
% \end{table*}

==> tables/main/tab_evaluation_strategies_vII.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{p{1.2cm}p{2.8cm}p{4.2cm}p{4.1cm}}
\toprule
\bf Type & \bf Metric &   \bf Measures  &  \textbf{Approximates} \\
\midrule
\multirow{3}{1cm}{Statistics}
&  Zipf Coefficient \citep{holtzman2019curious} & Unigram rank-frequency statistics & --
\\
& Self-BLEU  \citep{zhu2018texygen} & N-gram diversity  & --
\\
& Generation Perplexity \citep{fan2018heirarchical} & Generation quality via external model $R$& $|\mathbb{E}_Q [\log R(\xv)]-\mathbb{E}_P [\log R(\xv)]|$ (a single point inside $\Ccal(P, Q)$) \\
\midrule[0.03em]
\multirow{4}{1cm}{Language Modeling} &
Perplexity & Test-set perplexity & $\mathbb{E}_P [\log Q(\xv)]$\\
& $\epsilon$-perplexity \citep{martins2020sparse} & Perplexity w/ Laplace smoothing & $\mathbb{E}_P [\tilde{Q}(\xv)]$\\
& Sparsemax Score \citep{martins2020sparse} & LM quality (sparsemax loss~\cite{martins2016softmax}) & $\mathbb{E}_P [\tilde{Q}(\xv)]$ \\
& Token JS-Div. \citep{martins2020sparse} & LM quality (JS divergence)
& $\mathbb{E}_P [\tilde{Q}(\xv)]$\\
\midrule[0.03em]
Divergence Curve & {\name (this work)} &\begin{tabular}{l}Quality \& diversity via \\ the divergence curve \end{tabular} & $\Ccal(P,Q)$ at all $\lambda$\\
\bottomrule
\end{tabular}
\caption{\small{Summary of automatic distributional metrics for evaluating open-ended text generation. 
\name provides a summary of all points along the divergence curve, rather than a single point.
The summary is based on comparisons in a joint embedding space, rather than a statistic computed independently on each distribution.
% The expectations in the perplexity-based metrics are related to points on either extreme of the divergence curve.
% \name provides a summary of all points along this curve.
$\tilde{Q}$ informally refers to a quantity related to $Q$. 
% Note that JS divergence is measured at the token-level in \citep{martins2020sparse}.
}}
\label{tab:nlp:auto-metrics-survey}
% }
% \end{adjustbox}
\end{table*}


==> tables/main/tab_expt_tasks.tex <==
\begin{adjustbox}{max width=0.99\textwidth}
\begin{tabular}{llclrrr}
\toprule
\bf Task Domain & \bf Model & \bf Finetuning & \bf Dataset & 
\bf \begin{tabular}{r} Prompt \\ Length \end{tabular} & 
\bf \begin{tabular}{r} Max. \\ Generation \\ Length \end{tabular} & 
\bf \begin{tabular}{r} Number of \\ Generations \end{tabular} \\

\midrule

Web text & 
GPT-2 (all sizes) & 
 Pretrained  &
Webtext & $35$ tokens  & $1024$ tokens & $5000$
\\
News & 
Grover (all sizes)& 
Pretrained  & 
RealNews & varying & $1024$ tokens & $5000$
\\
Stories & GPT-2 medium & Finetuned &
WritingPrompts & $50$ tokens & $512$ tokens & $5000$ 
\\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables/new/fdiv_comparison.tex <==
\centering
\begin{adjustbox}{max width=0.8\linewidth}
\begin{tabular}{lccccccc}
\toprule
\begin{tabular}{c}
\textbf{Correlation}
\end{tabular} 
&  $\mauve_\kl$ &    $\fint_\kl$ &   $\midp_\kl$ &  $\mauve_{\chi^2}$ &  $\midp_{\chi^2}$ &        $\text{TV}$ &  $H^2$ \\
\midrule
$\mauve_\kl$ & 
  $1.0$ & $0.99$ &    $1.0$ &          $1.0$ &  $0.99$ & $1.0$ &       $1.0$ \\
BT/Human-like  &      $0.86$ &   $0.90$ &    $0.86$ &         $0.86$ &       $0.83$ &  $0.86$ &       $0.86$ \\
BT/Interesting &      $0.71$ &   $0.71$ &    $0.71$ &         $0.71$ &       $0.69$ &  $0.71$ &       $0.71$ \\
BT/Sensible    &      $0.76$ &   $0.79$ &    $0.76$ &         $0.76$ &       $0.76 $ &  $0.76$ &       $0.76$ \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables/new/ot_comparison.tex <==
%!TEX root = ../../main.tex


\centering
\begin{adjustbox}{max width=0.9 \linewidth}
\begin{tabular}{lcccccc}
\toprule

\multirow{3}{*}{\textbf{Correlation}}

& \multicolumn{3}{c}{OT variants}  & \multicolumn{3}{c}{\mauve variants} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
&  Plug-in &    Fr\'echet &   Quantized &  
\begin{tabular}{c} OT + \\ Linear \\ interpolation \end{tabular} &  
\begin{tabular}{c} OT + \\ Barycenteric \\ interpolation \end{tabular} &    
\begin{tabular}{c} KL + \\ Linear interp. \\ (default) \end{tabular} 
\\
\midrule
$\mauve_\kl$ & 
  $0.952$ & $0.996$ & $0.982$  & $0.985$  &  $0.982$  & $1.000$   \\
BT/Human-like  &     
  $0.810$  &  $0.857$  &  $0.810$  & $0.810$  &  $0.857$ & $0.857$ \\
BT/Interesting &      
  $0.714$ &   $0.714$ &    $0.714$ &         $0.714$ &       $0.714$ &  $0.714$  \\
BT/Sensible    &      $0.738$ &   $0.762$ &    $0.738$ &         $0.738$ &       $0.762$ &  $0.762$ \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables/related_work.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{p{1.2cm}p{2.8cm}p{4.2cm}p{4.1cm}}
\toprule
\bf Type & \bf Metric &   \bf Measures  &  \textbf{Approximates} \\
\midrule
\multirow{3}{1cm}{Statistics}
&  Zipf Coefficient \citep{holtzman2019curious} & Unigram rank-frequency statistics & --
\\
& Self-BLEU  \citep{zhu2018texygen} & N-gram diversity  & --
\\
& Generation Perplexity \citep{fan2018heirarchical} & Generation quality via external model $R$& $|\mathbb{E}_Q [\log R(\xv)]-\mathbb{E}_P [\log R(\xv)]|$ \\
\midrule[0.03em]
\multirow{4}{1cm}{Language Modeling} &
Perplexity & Test-set perplexity & $\mathbb{E}_P [\log Q(\xv)]$\\
& $\epsilon$-perplexity \citep{martins2020sparse} & Perplexity w/ Laplace smoothing & $\mathbb{E}_P [\tilde{Q}(\xv)]$\\
& Sparsemax Score \citep{martins2020sparse} & LM quality (sparsemax loss) & $\mathbb{E}_P [\tilde{Q}(\xv)]$ \\
& Token JS-Div. \citep{martins2020sparse} & LM quality (JS divergence)
& $\mathbb{E}_P [\tilde{Q}(\xv)]$\\
\midrule[0.03em]
Divergence Curve & {\name (this work)} &\begin{tabular}{l}Quality \& diversity via \\ the divergence curve \end{tabular} & $\Ccal(P,Q)$ at all $\lambda$\\
\bottomrule
\end{tabular}
\caption{\small{Summary of automatic distributional metrics for evaluating open-ended text generation. 
\name provides a summary of all points along the divergence curve, rather than a single point.
The summary is based on comparisons in a joint embedding space, rather than a statistic computed independently on each distribution.
% The expectations in the perplexity-based metrics are related to points on either extreme of the divergence curve.
% \name provides a summary of all points along this curve.
$\tilde{Q}$ informally refers to a quantity related to $Q$. 
\KP{TODO: beautify}
% Note that JS divergence is measured at the token-level in \citep{martins2020sparse}.
}}
\label{tab:nlp:auto-metrics-survey}
% }
% \end{adjustbox}
\end{table*}


==> tables_smooth/combined/beam_search.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Decoding}}
& \multirow{2}{*}{Greedy} & 
\multicolumn{2}{c}{Beam} 
& 
\multicolumn{2}{c}{Beam + no $4$-gram repeat}
& 
\multirow{2}{*}{Ancestral} & 
\multirow{2}{*}{Nucleus} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
& & $b=4$ & $b=8$ & $b=4$ & $b=8$ & & \\
\midrule
$\textbf{\mauve}^\star$ & 
$0.019$ & 
$0.040$ & 
$0.049$ & 
$0.438$ & 
$0.415$ & 
$0.655_{0.021}$ & 
\tabemph{} $\mathbf{0.906_{0.005}}$  \\
\bottomrule
\end{tabular}

==> tables_smooth/combined/corr_gold.tex <==
\begin{tabular}{llcccccc}
\toprule
\textbf{Metric} & \textbf{Task} & \textbf{Gen. PPL} & \textbf{Zipf Coef.} & \textbf{REP} & \textbf{Distinct-4} & \textbf{Self-BLEU} & \textbf{$\name^\star$} \\
\midrule
       Human-like/BT &      Web text &           $0.810$ &             $0.762$ &     $-0.500$ &             $0.738$ &            $0.500$ &        \tabemph{$\mathbf{0.857}$} \\
      Interesting/BT &      Web text &           $0.643$ &             $0.405$ &     $-0.571$ &             $0.524$ &            $0.262$ &        \tabemph{$\mathbf{0.714}$} \\
         Sensible/BT &      Web text &           $0.738$ &             $0.643$ &     $-0.476$ &             $0.595$ &            $0.452$ &        \tabemph{$\mathbf{0.762}$} \\
      Disc. Acc. &          News &           $0.468$ &             $0.595$ &      $0.792$ &             $0.653$ &            $0.516$ &        \tabemph{$\mathbf{0.956}$} \\
       % Disc. Acc. &       Stories &           $0.643$ &             $0.643$ &      $0.250$ &             $0.750$ &            $0.857$ &        \tabemph{$\mathbf{0.893}$} \\
       Disc. Acc. &       Stories &           $0.690$ & 	$0.762$ 	& $0.190$ & 	$0.833$ & 	\tabemph{$\mathbf{0.905}$} & 		\tabemph{$\mathbf{0.905}$} \\
       % 
       % $0.643$ &             $0.643$ &      $0.250$ &             $0.750$ &            $0.857$ &        \tabemph{$\mathbf{0.893}$} \\
\bottomrule
\end{tabular}



==> tables_smooth/combined/typical_decoding.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{
\textbf{Decoding}
}
& 
\multicolumn{6}{c}{Locally Typical Sampling}
& \multirow{2}{*}{Nucleus}\\
\cmidrule{2-7}
&
$\tau=0.2$ & $\tau=0.5$ & $\tau=0.7$ & $\tau=0.9$ & $\tau=0.95$ & $\tau=0.99$ &  
 \\
\midrule
$\textbf{\mauve}^\star$ & 
$0.862_{0.012}$ &
$0.896_{0.005}$ & 
$0.88_{0.01}$ & 
$0.939_{0.009}$ & 
$\tabemph{} \mathbf{0.950}_{0.005}$ & 
$0.914_{0.007}$ & 
$\tabemph{} \mathbf{0.952}_{0.003}$
% $0.826_{0.014}$ & 
% $0.868_{0.007}$ & 
% $0.850_{0.012}$ & 
% $0.920_{0.011}$ & 
% \tabemph{} $\mathbf{0.933_{0.007}}$ & 
% $0.889_{0.009}$ & 
% \tabemph{} $\mathbf{0.936_{0.004}}$  
\\
\bottomrule
\end{tabular}

==> tables_smooth/combined/webtext_full_LM.tex <==
\begin{tabular}{llrrrrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &  \bf   SP($\uparrow$) &  \bf JS($\downarrow$) & \bf $\epsilon$-PPL($\downarrow$) & \bf Human/BT($\uparrow$) & \bf $\mauve^\star$($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Greedy &                         $0.431$ &           $0.394$ &                   $1049.589$ &          --            &                    $0.019$ \\
& Sampling &             $0.653$ &           $0.425$ &                     $19.401$ &             $-27.52$ &            $0.655_{0.018}$ \\
      & Nucleus, $0.9$ &         $0.652$ &           $0.414$ &                     $25.938$ &             $-15.78$ &            $0.906_{0.005}$ \\
\midrule
\multirow{4}{*}{medium} & Greedy &                          $0.465$ &           $0.371$ &                    $708.057$ &              --        &                    $0.024$ \\
& Sampling &      $0.670$ &           $0.402$ &                     $14.631$ &             $-30.77$ &            $0.446_{0.010}$ \\
      & Nucleus, $0.9$ &              $0.670$ &           $0.391$ &                     $18.821$ &              $-3.43$ &            $0.936_{0.004}$ \\
\midrule
\multirow{4}{*}{large} & Greedy &                     $0.483$ &           $0.359$ &                    $580.020$ &            --          &                    $0.026$ \\
& Sampling &     $0.679$ &           $0.381$ &                     $12.658$ &              $-6.93$ &            $0.878_{0.008}$ \\
      & Nucleus, $0.95$ &    $0.679$ &           $0.374$ &                     $14.938$ &              $12.55$ &            $0.952_{0.002}$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Greedy &                      $0.496$ &  \tabemph{$\mathbf{0.349}$} &                    $497.696$ &              --        &                    $0.033$ \\
    & Sampling &      \tabemph{$\mathbf{0.686}$} &           $0.369$ &            \tabemph{$\mathbf{11.412}$} &               $8.97$ &            $0.908_{0.005}$ \\
      & Nucleus, $0.95$ &            $0.686$ &           $0.363$ &                     $13.677$ &    \tabemph{$\mathbf{15.66}$} &   \tabemph{$\mathbf{0.955}_{0.004}$} \\
      & Adversarial &           n/a &           n/a &                     n/a &             -- &            $0.057$ \\
\bottomrule
\end{tabular}


==> tables_smooth/combined/webtext_full_ref.tex <==
\begin{tabular}{lllllllrl}
\toprule
\bf GPT-2  Size    &   \bf    Decoding             &      \bf              Gen. PPL &           \bf     Zipf Coef. &               \bf        Rep. &       \bf         Distinct-4 &           \bf      Self-BLEU & \bf Human($\uparrow$) & \bf $\mauve^\star$ ($\uparrow$) \\
\midrule
\multirow{4}{*}{small} & Sampling &          $101.880_{0.627}$ &           $0.926_{0.001}$ &           $0.001_{0.000}$ &           $0.941_{0.001}$ &           $0.327_{0.003}$ &                      $-27.52$ &            $0.655_{0.018}$ \\
% $0.589_{0.018}$ \\
      & Greedy &                    $1.224$ &                   $1.037$ &                   $0.942$ &                   $0.072$ &           $0.465_{0.000}$ &                 --            &                   $0.019$ \\
      % $0.008$ \\
      & Nucleus, $0.9$ &           $23.788_{0.144}$ &           $1.012_{0.002}$ &           $0.010_{0.001}$ &           $0.859_{0.002}$ &           $0.436_{0.004}$ &              $-15.78$ &            $0.906_{0.005}$ \\
      % $0.878_{0.006}$ \\
      & Adversarial &            \tabemph{$\mathbf{12.554}$} &           $1.073$ &           $0.006$ &           $0.365$ &           $0.525$ &             -- &            $0.043$ \\
\midrule
\multirow{4}{*}{medium} & Sampling &          $129.263_{0.798}$ &           $0.872_{0.001}$ &           $0.001_{0.000}$ &           $0.953_{0.001}$ &           $0.281_{0.002}$ &              $-30.77$ &           $0.446_{0.010}$ \\
% $0.373_{0.010}$ \\
      & Greedy &                    $1.241$ &                   $0.978$ &                   $0.903$ &                   $0.091$ &                   $0.415$ &                 --        &                    $0.024$ \\
      % $0.012$ \\
      & Nucleus, $0.9$ &           $21.073_{0.134}$ &           \tabemph{$\mathbf{0.957}_{0.001}$} &           $0.005_{0.001}$ &  \tabemph{$\mathbf{0.884}_{0.001}$} &  \tabemph{$\mathbf{0.402}_{0.003}$} &                  $-3.43$ &            $0.936_{0.004}$ \\
      % $0.915_{0.006}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $1.006$ &           $0.005$ &           $0.381$ &           $0.444$ &            -- &            $0.044$ \\
\midrule
\multirow{4}{*}{large} & Sampling &           $30.080_{0.196}$ &           $0.930_{0.002}$ &  \tabemph{$\mathbf{0.002}_{0.001}$} &           $0.916_{0.001}$ &           $0.358_{0.001}$ &                $-6.93$ &         $0.878_{0.008}$ \\
% $0.845_{0.010}$ \\
      & Greedy &                    $1.232$ &                   $0.983$ &                   $0.881$ &                   $0.100$ &                   $0.413$ &       --          &                    $0.026$ \\
      % $0.012$ \\
      & Nucleus, $0.95$ &  $13.499_{0.058}$ &  $0.967_{0.002}$ &           $0.006_{0.001}$ &           $0.870_{0.001}$ &           $0.412_{0.002}$ &             $12.55$ &            $0.952_{0.002}$ \\
      % $0.936_{0.003}$ \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.965$ &           $0.005$ &           $0.395$ &           $0.429$ &        -- &            $0.035$ \\
\midrule[0.03em]
\multirow{4}{*}{xl} & Sampling &           $31.886_{0.447}$ &           $0.930_{0.001}$ &           $0.002_{0.001}$ &           $0.913_{0.001}$ &           $0.360_{0.003}$ &            $8.97$ &            $0.908_{0.005}$ \\
% $0.882_{0.006}$ \\
      & Greedy &                    $1.278$ &                   $0.975$ &                   $0.859$ &                   $0.115$ &                   $0.417$ &               --        &                    $0.033$ \\
      & Nucleus, $0.95$ &           $14.143_{0.043}$ &           $0.966_{0.002}$ &           $0.005_{0.000}$ &           $0.868_{0.001}$ &           $0.413_{0.002}$ &      \tabemph{$\mathbf{15.66}$} &   
      \tabemph{$\mathbf{0.955_{0.004}}$} \\
      % \tabemph{$\mathbf{0.940}_{0.006}$} \\
      & Adversarial &           \tabemph{$\mathbf{12.554}$} &           $0.986$ &           $0.005$ &           $0.397$ &           $0.448$ &      -- &            $0.057$ \\
\midrule
Human &         n/a          &                   $12.602$ &                   $0.952$ &                   $0.002$ &                   $0.878$ &                   $0.382$ &         $47.25$ &            --                \\
\bottomrule
\end{tabular}


==> tables_smooth/combined/wp_std.tex <==
\begin{tabular}{llllllll}
\toprule
\textbf{Decoding} &                   \textbf{Gen. PPL} &                \textbf{Zipf Coef.} &                       \textbf{REP} &                \textbf{Distinct-4} &                 \textbf{Self-BLEU} & \textbf{\% Disc. Acc. ($\downarrow$)} & $\textbf{\mauve}^\star(\uparrow)$ \\
\midrule
Sampling & $38.983_{0.143}$ & $\tabemph{}  \mathbf{1.066}_{0.002}$ & $\tabemph{}  \mathbf{0.001}_{0.000}$ & $0.833_{0.001}$ & $0.518_{0.003}$ & $78.098_{0.365}$ & $0.929_{0.007}$ \\
Nucleus, $0.9$ & $15.433_{0.042}$ & $1.201_{0.002}$ & $0.006_{0.001}$ & $0.719_{0.001}$ & $0.637_{0.002}$ & $75.150_{0.373}$ & $0.914_{0.005}$ \\
Nucleus, $0.92$ & $17.422_{0.060}$ & $1.179_{0.002}$ & $0.004_{0.001}$ & $0.742_{0.001}$ & $0.620_{0.003}$ & $71.979_{0.594}$ & $0.926_{0.003}$ \\
Nucleus, $0.95$ & $\tabemph{}  \mathbf{21.599}_{0.127}$ & $1.147_{0.002}$ & $0.003_{0.000}$ & $\tabemph{}  \mathbf{0.775}_{0.002}$ & $0.589_{0.005}$ & $\tabemph{}  \mathbf{68.586}_{0.583}$ & $\tabemph{}  \mathbf{0.940}_{0.003}$ \\
Top-$50$ & $13.735_{0.027}$ & $1.293_{0.004}$ & $0.002_{0.000}$ & $0.706_{0.001}$ & $0.664_{0.003}$ & $83.549_{0.381}$ & $0.886_{0.010}$ \\
Top-$100$ & $16.527_{0.041}$ & $1.252_{0.001}$ & $0.002_{0.000}$ & $0.743_{0.001}$ & $0.631_{0.001}$ & $78.150_{0.207}$ & $0.913_{0.005}$ \\
Top-$500$ & $23.833_{0.076}$ & $1.153_{0.001}$ & $0.001_{0.000}$ & $0.794_{0.001}$ & $\tabemph{}  \mathbf{0.576}_{0.002}$ & $69.680_{0.450}$ & $\tabemph{}  \mathbf{0.942}_{0.004}$ \\
Greedy & $1.739$ & $1.362$ & $0.988$ & $0.101$ & $0.742$ & $99.712$ & $0.013$ \\
\midrule
Human             &                   $19.704$ &                   $1.101$ &                   $0.001$ &                   $0.783$ &                   $0.571$ &                              &                            \\
\bottomrule
\end{tabular}



==> tables_smooth/grover/main_grover.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
\bf Grover Size      &    \bf  Decoding              &       \bf     Gen. PPL &     \bf    Zipf Coef. &     \bf           Rep. &    \bf     Distinct-4 &      \bf    Self-BLEU &  \bf \% Disc. Acc.($\downarrow$) & \bf $\mauve^\star$($\uparrow$) \\
\midrule
\multirow{3}{*}{base} & Sampling &           $37.505$ &           $0.942$ &           $0.002$ &           $0.882$ &           $0.419$ &                     $99.925$ &                    $0.754$ \\
      & Greedy &            $1.413$ &           $1.038$ &           $0.518$ &           $0.081$ &           $0.548$ &                    $100.000$ &                    $0.012$ \\
      & Nucleus, $0.96$ &           $23.064$ &           $0.974$ &           $0.006$ &  \tabemph{$\mathbf{0.847}$} &           $0.462$ &                     $99.950$ &                    $0.764$ \\
\midrule[0.03em]
\multirow{3}{*}{large} & Sampling &           $27.796$ &  ${0.946}$ &  \tabemph{$\mathbf{0.002}$} &           $0.878$ &           $0.429$ &                     $99.450$ &                    $0.836$ \\
      & Greedy &            $1.575$ &           $1.012$ &           $0.366$ &           $0.124$ &           $0.504$ &                    $100.000$ &                    $0.013$ \\
      & Nucleus, $0.98$ &           $20.792$ &           \tabemph{$\mathbf{0.962}$} &           $0.002$ &           $0.859$ &           $0.450$ &                     $98.475$ &                    $0.800$ \\
\midrule[0.03em]
\multirow{3}{*}{mega} & Sampling &           $22.656$ &           $0.950$ &           $0.001$ &           $0.879$ &           $0.427$ &                     $97.300$ &                    $0.847$ \\
      & Greedy &            $1.796$ &           $1.003$ &           $0.316$ &           $0.176$ &           $0.500$ &                    $100.000$ &                    $0.013$ \\
      & Nucleus, $0.96$ &  \tabemph{$\mathbf{14.834}$} &           $0.972$ &           $0.003$ &           $0.848$ &  \tabemph{$\mathbf{0.469}$} &            \tabemph{$\mathbf{88.675}$} &           \tabemph{$\mathbf{0.852}$} \\
\midrule
Human &      n/a             &           $15.356$ &           $0.956$ &           $0.002$ &           $0.842$ &           $0.473$ &         --                     &        --                    \\
\bottomrule
\end{tabular}


==> tables_smooth/new/fdiv_comparison.tex <==
\centering
\begin{adjustbox}{max width=0.8\linewidth}
\begin{tabular}{lccccccc}
\toprule
\begin{tabular}{c}
\textbf{Correlation}
\end{tabular} 
&  $\mauve_\kl^\star$ &    $\fint_\kl^\star$ &   $\midp_\kl^\star$ &  $\mauve_{\chi^2}^\star$ &  $\midp_{\chi^2}^\star$ &        $\text{TV}^\star$ &  $H^2_\star$ \\
\midrule
$\mauve_\kl^\star$ & 
  $1.0$ & $0.99$ &    $1.0$ &          $1.0$ &  $1.0$ & $1.0$ &       $1.0$ \\
BT/Human-like & $0.857$ & \tabemph{} $\mathbf{0.929}$ & $0.857$ & $0.857$ & $0.857$ & $0.857$ & $0.857$ \\
BT/Interesting & $0.714$ & \tabemph{} $\mathbf{0.738}$ & $0.714$ & $0.714$ & $0.714$ & $0.714$ & $0.714$ \\
BT/Sensible & $0.762$ & \tabemph{} $\mathbf{0.833}$ & $0.762$ & $0.762$ & $0.762$ & $0.762$ & $0.762$ \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables_smooth/new/fdiv_full.tex <==
\begin{tabular}{ccrrrrrrrr}
 \toprule
\begin{tabular}{c} \textbf{GPT-2} \\  \textbf{Size}\end{tabular}
 &  \textbf{Decoding} & 
 ${\mauve}_\kl^\star$ ($\uparrow$) &    $\fint_\kl^\star$ ($\downarrow$) &   $\midp_\kl^\star$ ($\downarrow$) &  $\mauve_{\chi^2}^\star$ ($\uparrow$) &  $\midp_{\chi^2}^\star$ ($\downarrow$) &        ${\tv}^\star$ ($\downarrow$) &  $H^2_\star$ ($\downarrow$) & 
 % \textbf{BT/Human-like} ($\uparrow$) 
 \begin{tabular}{c}\textbf{BT} ($\uparrow$) \\ \textbf{Human-like}  \end{tabular}
 \\
 % $\textbf{\mauve}_\kl^\star$ &    $\textbf{\fint}_\kl^\star$ &   $\textbf{\midp}_\kl^\star$ &  $\textbf{\mauve}_{\chi^2}^\star$ &  $\textbf{\midp}_{\chi^2}^\star$ &        $\textbf{TV}^\star$ &  $\mathbf{H^2}_\star$ & \textbf{BT/Human-like} \\
 \midrule
\multirow[c]{2}{*}{small} & Sampling & $0.655_{0.018}$ & $0.033_{0.002}$ & $0.105_{0.004}$ & $0.335_{0.020}$ & $0.191_{0.007}$ & $0.363_{0.006}$ & $0.225_{0.010}$ & $-27.518$ \\
 & Nucleus, $0.9$ & $0.906_{0.005}$ & $0.016_{0.001}$ & $0.044_{0.001}$ & $0.734_{0.011}$ & $0.084_{0.003}$ & $0.230_{0.005}$ & $0.091_{0.003}$ & $-15.783$ \\
 \hline
\multirow[c]{2}{*}{medium} & Sampling & $0.446_{0.010}$ & $0.042_{0.001}$ & $0.160_{0.003}$ & $0.164_{0.004}$ & $0.277_{0.003}$ & $0.443_{0.004}$ & $0.356_{0.009}$ & $-30.769$ \\
 & Nucleus, $0.9$ & $0.936_{0.004}$ & $0.012_{0.001}$ & $0.035_{0.001}$ & $0.805_{0.009}$ & $0.068_{0.002}$ & $0.205_{0.004}$ & $0.073_{0.002}$ & $-3.429$ \\
 \hline
\multirow[c]{2}{*}{large} & Sampling & $0.878_{0.008}$ & $0.017_{0.000}$ & $0.052_{0.002}$ & $0.672_{0.016}$ & $0.098_{0.003}$ & $0.251_{0.004}$ & $0.107_{0.004}$ & $-6.935$ \\
 & Nucleus, $0.95$ & $0.952_{0.002}$ & $0.010_{0.000}$ & $0.030_{0.001}$ & $0.849_{0.007}$ & $0.058_{0.002}$ & $0.187_{0.005}$ & $0.061_{0.002}$ & $12.553$ \\
 \hline
\multirow[c]{2}{*}{xl} & Sampling & $0.908_{0.005}$ & $0.014_{0.001}$ & $0.044_{0.001}$ & $0.737_{0.012}$ & $0.083_{0.003}$ & $0.232_{0.005}$ & $0.090_{0.003}$ & $8.966$ \\
 & Nucleus, $0.95$ & $\tabemph{}  \mathbf{0.955}_{0.004}$ & $\tabemph{}  \mathbf{0.010}_{0.001}$ & $\tabemph{}  \mathbf{0.029}_{0.002}$ & $\tabemph{}  \mathbf{0.857}_{0.012}$ & $\tabemph{}  \mathbf{0.056}_{0.003}$ & $\tabemph{}  \mathbf{0.185}_{0.006}$ & $\tabemph{}  \mathbf{0.059}_{0.003}$ & $\tabemph{}  \mathbf{15.664}$ \\
\bottomrule
\end{tabular}

==> tables_smooth/new/non-deep-embedding.tex <==
\begin{adjustbox}{max width=0.9\linewidth}
\renewcommand{\arraystretch}{1.2}
\small
    \begin{tabular}{ccccc}
    \toprule
        \textbf{Correlation} & 
        \textbf{GPT-2 Embedding} & 
        \textbf{GloVe Embedding} &
        \textbf{$N$-gram Kernel} &
        \textbf{Subsequence Kernel} \\
        \midrule
    $\mauve_\kl^\star$ (default) &
    $1.00$ & $0.993$ & $0.727$ & $0.783$
    \\
    BT/Human-like & 
    $0.857$ &	$0.928$ & $0.500$ & $0.286$
    \\
    BT/Interesting &
    $0.714$ & $0.738$ & $0.262$ & $0.214$
    \\
    BT/Sensible &
    $0.762$ & $0.833$ & $0.429$ & $0.214$
    \\
    \bottomrule
    \end{tabular}
\end{adjustbox}

==> tables_smooth/new/ot_comparison.tex <==
%!TEX root = ../../main.tex


\centering
\begin{adjustbox}{max width=0.9 \linewidth}
\begin{tabular}{lcccccc}
\toprule

\multirow{3}{*}{\textbf{Correlation}}

& \multicolumn{3}{c}{\textbf{OT variants}}  & \multicolumn{3}{c}{\textbf{\mauve variants}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
&  Plug-in &    Fr\'echet &   Quantized &  
\begin{tabular}{c} OT + \\ Linear \\ interpolation \end{tabular} &  
\begin{tabular}{c} OT + \\ Barycenteric \\ interpolation \end{tabular} &    
\begin{tabular}{c} (Default) KL + \\ Linear \\ interpolation  \end{tabular} 
\\
\midrule
$\mauve_\kl^\star$ & 
  $0.954$ & $0.997$ & $0.980$  & $0.983$  &  $0.980$  & $1.000$   \\
BT/Human-like  &     
  $0.810$  &  $0.857$  &  $0.810$  & $0.810$  &  $0.857$ & $0.857$ \\
BT/Interesting &      
  $0.714$ &   $0.714$ &    $0.714$ &         $0.714$ &       $0.714$ &  $0.714$  \\
BT/Sensible    &      $0.738$ &   $0.762$ &    $0.738$ &         $0.738$ &       $0.762$ &  $0.762$ \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables_smooth/new/ot_full.tex <==
% \renewcommand*{\arraystretch}{1.2}
\begin{tabular}{ccrrrrrrr}
\toprule
 % &  & w2_continuous & frechet & w2_discrete & w2_mauve & barycenter_w2_mauve & mauve-kmeans & BT/Human-like \\
\multirow{3}{*}{
\begin{tabular}{c}
\textbf{GPT-2} \\
\textbf{Size}
\end{tabular}
} & 
\multirow{3}{*}{\textbf{Decoding}} & \multicolumn{3}{c}{\textbf{OT variants} ($\downarrow)$}  & \multicolumn{3}{c}{\textbf{\mauve variants} ($\uparrow$)} & \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} 
& &  Plug-in &    Fr\'echet &   Quantized &  
\begin{tabular}{c} OT + \\ Linear \\ interpolation \end{tabular} &  
\begin{tabular}{c} OT + \\ Barycenteric \\ interpolation \end{tabular} &    
\begin{tabular}{c} (Default) KL + \\ Linear \\ interpolation  \end{tabular}  &
% \textbf{BT/Human-like} ($\uparrow$)
 \begin{tabular}{c} \textbf{BT} ($\uparrow$) \\ \textbf{Human-like} \end{tabular}
\\
\midrule
\multirow[c]{2}{*}{small} & Sampling & $763.281_{1.264}$ & $199.591_{0.788}$ & $0.158_{0.001}$ & $0.814_{0.001}$ & $0.937_{0.001}$ & $0.655_{0.018}$ & $-27.518$ \\
 & Nucleus, $0.9$ & $693.263_{4.610}$ & $148.388_{1.236}$ & $0.083_{0.005}$ & $0.935_{0.007}$ & $0.964_{0.001}$ & $0.906_{0.005}$ & $-15.783$ \\
 \midrule
\multirow[c]{2}{*}{medium} & Sampling & $791.758_{4.780}$ & $224.970_{2.526}$ & $0.208_{0.002}$ & ${0.725}_{0.004}$ & ${0.914}_{0.001}$ & ${0.446}_{0.010}$ & ${-30.769}$ \\
 & Nucleus, $0.9$ & $700.496_{3.961}$ & $140.174_{0.813}$ & $0.077_{0.004}$ & $0.942_{0.005}$ & $0.967_{0.001}$ & $0.936_{0.004}$ & $-3.429$ \\
 \midrule
\multirow[c]{2}{*}{large} & Sampling & $717.909_{5.618}$ & $153.358_{1.325}$ & $0.104_{0.004}$ & $0.905_{0.006}$ & $0.958_{0.002}$ & $0.878_{0.008}$ & $-6.935$ \\
 & Nucleus, $0.95$ & $\tabemph{} \mathbf{681.883}_{4.367}$ & $133.583_{0.762}$ & $0.062_{0.001}$ & $0.961_{0.002}$ & $0.969_{0.001}$ & $0.952_{0.002}$ & $12.553$ \\
 \midrule
\multirow[c]{2}{*}{xl} & Sampling & $705.482_{4.617}$ & $146.593_{1.136}$ & $0.090_{0.003}$ & $0.924_{0.004}$ & $0.962_{0.001}$ & $0.908_{0.005}$ & $8.966$ \\
 & Nucleus, $0.95$ & $685.131_{3.258}$ & $\tabemph{} \mathbf{132.927}_{1.555}$ & $\tabemph{} \mathbf{0.061}_{0.003}$ & $\tabemph{} \mathbf{0.962}_{0.004}$ & $\tabemph{} \mathbf{0.970}_{0.001}$ & $\tabemph{} \mathbf{0.955}_{0.004}$ & $\tabemph{} \mathbf{15.664}$ \\
\bottomrule
\end{tabular}

==> tables_smooth/new/smoothing.tex <==
\begin{tabular}{ccrrrr}
\toprule
 \multirow[c]{2}{*}{\textbf{GPT-2 Size}}&   
 \multirow[c]{2}{*}{\textbf{Decoding}} &  \multicolumn{2}{c}{\textbf{\mauve} ($\uparrow$)}  & 
 \multicolumn{2}{c}{\textbf{Empty bins}}
 \\
 \cmidrule(lr){3-4} \cmidrule(lr){5-6}
 & & No Smoothing  & K-T Smoothing & Total Number & Percentage \\
 \midrule
\multirow[c]{3}{*}{small} & Sampling & $0.589_{0.018}$ & $0.655_{0.018}$ & $54.2_{6.6}$ & $5.4_{0.7}$ \\
 & Greedy & $0.008$ & $0.019_{0.000}$ & $373.0$ & $37.3$ \\
 & Nucleus, $0.9$ & $0.878_{0.006}$ & $0.906_{0.005}$ & $36.4_{4.9}$ & $3.6_{0.5}$ \\
 \midrule
\multirow[c]{3}{*}{medium} & Sampling & $0.373_{0.010}$ & $0.446_{0.010}$ & $77.0_{5.5}$ & $7.7_{0.5}$ \\
 & Greedy & $0.012$ & $0.024$ & $314.0$ & $31.4$ \\
 & Nucleus, $0.9$ & $0.915_{0.006}$ & $0.936_{0.004}$ & $29.0_{6.6}$ & $2.9_{0.7}$ \\
 \midrule
\multirow[c]{3}{*}{large} & Sampling & $0.845_{0.010}$ & $0.878_{0.008}$ & $30.2_{1.3}$ & $3.0_{0.1}$ \\
 & Greedy & $0.012_{0.000}$ & $0.026_{0.000}$ & $311.4_{0.8}$ & $31.1_{0.1}$ \\
 & Nucleus, $0.95$ & $0.936_{0.003}$ & $0.952_{0.002}$ & $26.6_{3.0}$ & $2.7_{0.3}$ \\
 \midrule
\multirow[c]{3}{*}{xl} & Sampling & $0.882_{0.006}$ & $0.908_{0.005}$ & $27.6_{6.8}$ & $2.8_{0.7}$ \\
 & Greedy & $0.016$ & $0.033$ & $288.0$ & $28.8$ \\
 & Nucleus, $0.95$ & $\tabemph{} \mathbf{0.940}_{0.006}$ & $\tabemph{} \mathbf{0.955}_{0.004}$ & $23.4_{2.9}$ & $2.3_{0.3}$ \\

 \bottomrule
\end{tabular}

